GraphSense: A General-Purpose Cryptoasset Analytics Platform

There is currently an increasing demand for cryptoasset analysis tools among cryptoasset service providers, the financial industry in general, as well as across academic fields. At the moment, one can choose between commercial services or low-level open-source tools providing programmatic access. In this paper, we present the design and implementation of another option: the GraphSense Cryptoasset Analytics Platform, which can be used for interactive investigations of monetary flows and, more importantly, for executing advanced analytics tasks using a standard data science tool stack. By providing a growing set of open-source components, GraphSense could ultimately become an instrument for scientific investigations in academia and a possible response to emerging compliance and regulation challenges for businesses and organizations dealing with cryptoassets.

==> sections/acknowledgment.tex <==
% !TeX root = ../main.tex

\section{Acknowledgment}

We would like to thank Roman Karl, Mihai Bartha and Abraham Hinteregger for their contributions to GraphSense. In recent years, work on GraphSense has partially been funded by the Austrian security research program KIRAS of the Federal Ministry of
Agriculture, Regions and Tourism (BMLRT) under the project VIRTCRIME (No. 860672) and KRYPTOMONITOR (No. 879686) and, inter alia, by the European Union’s Horizon 2020 research and innovation program under the project TITANIUM (No. 740558).
